On Code-Induced Reasoning in LLMs

Code data has been shown to enhance the reasoning capabilities of large language models (LLMs), but it remains unclear which aspects of code are most responsible. We investigate this question with a systematic, data-centric framework. We construct parallel instruction datasets in ten programming languages and apply controlled perturbations that selectively disrupt structural or semantic properties of code. We then finetune LLMs from five model families and eight scales on each variant and evaluate their performance on natural language, math, and code tasks. Across 3,331 experiments, our results show that LLMs are more vulnerable to structural perturbations than semantic ones, particularly on math and code tasks. Appropriate abstractions like pseudocode and flowcharts can be as effective as code, while encoding the same information with fewer tokens without adhering to original syntax can often retain or even improve performance. Remarkably, even corrupted code with misleading signals remains competitive when surface-level regularities persist. Finally, syntactic styles also shape task-specific gains with Python favoring natural language reasoning and lower-level languages such as Java and Rust favoring math. Through our systematic framework, we aim to provide insight into how different properties of code influence reasoning and inform the design of training data for enhancing LLM reasoning capabilities.

==> figures/prompts/normal_code.tex <==
\begin{figure*}[h]
    \centering
        \tcbset{
  colframe=black!80,   % lighter border
  colback=gray!9,      % lighter background
  arc=4mm,             % slightly softer corners
  boxrule=0.8pt,       % thinner border line
  fonttitle=\bfseries, % bold if you use titles
  fontupper=\large     % larger font size for content
}
    \begin{tcolorbox}
    \tiny
    \textbf{You are tasked with generating code based on a specified programming language and instruction.} Your goal is to generate code that follows the syntax and semantics of the specified language. If the instruction is invalid (e.g., contradicts the language's rules or references functions or constructs from a different language), you must strictly respond with \textbf{"invalid."}

    \textbf{Guidelines:}
    - \textbf{Valid Code:}
       - The generated code must be syntactically and semantically correct according to the specified language.
       - The code should follow standard conventions and best practices for the given language.
       - Do \textbf{not} provide any explanation for valid code — only output the code itself.

    - \textbf{Invalid Instruction:}
       - If the instruction references constructs, functions, or syntax not supported by the specified language, respond with `"invalid"`.
       - Do \textbf{not} attempt to correct the invalid instruction — just respond with `"invalid"`.
       - Do \textbf{not} provide a reason or explanation for why the instruction is invalid.

    \textbf{Examples:}

    \textbf{Example 1:}
    Instruction: "Write a function to convert a list to a set."
    Language: Python
    Response:
    \begin{verbatim}
    def list_to_set(input_list):
        return set(input_list)
    \end{verbatim}

    \textbf{Example 2:}
    Instruction: "Create a class with a method that prints 'Hello' using console.log()."
    Language: Python
    Response: invalid

    \textbf{Example 3:}
    Instruction: "List all files, including hidden ones, in the current directory."
    Language: Shell
    Response: ls -a

    \textbf{Example 4:}
    Instruction: "Define a function using 'def' that returns the length of a string."
    Language: JavaScript
    Response: invalid

    \textbf{Instruction:}
    If the instruction is valid, output the code directly (without explanations).
    If the instruction is invalid, respond with "invalid" (no explanation).

    \textbf{Input:}
    Instruction: \{instruction\}
    Language: \{language\}

    \textbf{Output:}
    \{\{response\}\}
    \end{tcolorbox}
    \caption{Code generation prompt. The task is to generate valid code for a given language or respond with "invalid" if the instruction contradicts the language's rules.}
    \label{fig:normal_code_prompt}
\end{figure*}

==> tables/rubrics.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{lll}
% \toprule
% \textbf{Language} & \textbf{Prompt} & \textbf{Rubric} \\
% \midrule

% CPP &
% \begin{tabular}[c]{@{}l@{}}/*\\ 
% \n\\ Insert a number \\ \"\\ delimeter\\ \"\\  between every two consecutive elements of input vector `numbers\\ \"\n\\ 
% >>> intersperse({}, 4)\\ 
% \n\\ {}\\ 
% \n\\ >>> intersperse({1, 2, 3}, 4)\\ 
% \n\\ {1, 4, 2, 4, 3}\\ 
% \n\\ */\\ 
% \n\\ \#include<stdio.h>\\ 
% \n\\ \#include<vector>\\ 
% \n\\ using namespace std;\\ 
% \n\\ vector<int> intersperse(vector<int> numbers, int delimeter){ \\ \n
% \end{tabular} &
% \begin{tabular}[c]{@{}l@{}}### Evaluation Rubric for the `intersperse` Function Implementation\\ \n
% **Score 1**: The response is completely irrelevant or nonsensical, failing to implement any functionality related to the prompt. For example, it might return a completely different data type or structure that does not resemble a vector of integers.\\ \n
% **Score 2**: The response attempts to define a function named `intersperse` but contains major syntax errors or logical flaws that prevent it from compiling or running at all. For instance, it could have incorrect parameter types or fail to include necessary headers.\\ \n
% **Score 3**: The response includes some code that resembles the intended functionality but is fundamentally incorrect. It may not handle edge cases like an empty vector properly or fails to return the correct output format, such as returning a vector but not interspersing the delimiter correctly.\\ \n
% **Score 4**: The response shows an attempt to implement the `intersperse` function but only partially addresses the task. It may handle non-empty vectors correctly but fails to return the correct output for the empty vector test case or uses an incorrect approach to add delimiters.\\ \n
% **Score 5**: The response correctly defines the `intersperse` function and handles the basic case of a non-empty vector. However, it may not pass all test cases, such as failing to intersperse the delimiter correctly between all elements or mishandling edge cases.\\ \n
% **Score 6**: The response is mostly correct but has minor flaws. It might pass the test case for an empty vector but incorrectly handle cases with more than one element. For example, it might intersperse delimiters correctly but return an extra delimiter at the end or begin with one.\\ \n
% **Score 7**: The response correctly implements the `intersperse` function and passes most of the test cases provided. However, it may still have a minor issue that prevents it from being fully correct, such as not handling specific edge cases or producing an unexpected output format.\\ \n
% **Score 8**: The response closely aligns with the canonical solution and passes all the test cases. It correctly intersperses the delimiter for non-empty vectors and handles the empty vector case properly. Minor improvements could be made in code style or efficiency, but the logic is sound.\\ \n
% **Score 9**: The response is almost identical to the canonical solution, passing all test cases without any issues. It may include slight differences in implementation style, such as variable naming or formatting, but does not affect the correctness of the output.\\ \n
% **Score 10**: The response perfectly implements the `intersperse` function as described in the prompt. It passes all test cases, including edge cases, and adheres to best practices in coding style and efficiency, matching the canonical solution exactly.
% \end{tabular} \\

% \midrule
% GO &
% \begin{tabular}[c]{@{}l@{}}// Insert a number 'delimeter' between every two consecutive elements of input list `numbers'\\ 
% // >>> Intersperse([], 4)\\ 
% // []\\ 
% // >>> Intersperse([1, 2, 3], 4)\\ 
% // [1, 4, 2, 4, 3]\\ 
% func Intersperse(numbers []int, delimeter int) []int {\\ 
% \end{tabular} &
% \begin{tabular}[c]{@{}l@{}}### Evaluation Rubric for Intersperse Function\\ \n
% **Score 1:** The response is irrelevant or completely nonsensical, failing to implement any part of the required functionality. For example, returning a string or unrelated data type instead of a slice of integers.\\ \n
% **Score 2:** The response shows minimal effort, perhaps returning a hardcoded value or an empty slice without any logic implemented. For instance, returning `[]int{}` regardless of the input.\\ \n
% **Score 3:** The response attempts to implement the function but does not follow the prompt requirements. It may include a loop or condition but fails to correctly intersperse the delimiter or handle edge cases, such as returning just the input list without modification.\\ \n
% **Score 4:** The response provides a partial implementation that intersperses the delimiter for some cases but fails on others. For example, it may correctly handle non-empty lists but return an incorrect result for an empty list or use the wrong delimiter.\\ \n
% **Score 5:** The response implements the basic functionality, correctly interspersing the delimiter for simple cases but may fail on edge cases or have minor logical errors. For example, it might correctly handle `[1, 2, 3]` but not return `[]` for an empty input list.\\ \n
% **Score 6:** The response correctly intersperses the delimiter for non-empty lists but may not handle all test cases correctly. It could return the correct output for some test cases, like `[5, 6, 3, 2]`, but fail for others, such as returning the wrong result for `[]` or `[2, 2, 2]`.\\ \n
% **Score 7:** The response is mostly correct, passing most test cases but with minor flaws or inefficiencies. For instance, it may pass the test cases for non-empty lists but still not return the correct output for an empty list, demonstrating an understanding of the prompt with small errors.\\ \n
% **Score 8:** The response is nearly complete, correctly handling all provided test cases except for one minor edge case or inefficiency in the logic. It may pass all non-empty tests and return the correct empty list but could have a slight performance issue or redundancy in the code.\\ \n
% **Score 9:** The response is almost fully correct, aligning very closely with the canonical solution. It passes all provided test cases, including edge cases, but may have a minor stylistic or efficiency issue, such as using a less optimal method for appending to the result slice.\\ \n
% **Score 10:** The response is fully correct, implementing the functionality as specified in the prompt, matching the canonical solution exactly, and passing all test cases, including edge cases. The logic is clear, efficient, and adheres to best practices in Go programming.
% \end{tabular} \\

% \midrule
% Java &
% \begin{tabular}[c]{@{}l@{}}import java.util.*;\\ 
% \n\\ import java.lang.*;\\ 
% \n\n\\ class Solution {\\ 
% \n\\     /**\\ 
% \n\\     Return list of all prefixes from shortest to longest of the input string\\ 
% \n\\     >>> allPrefixes(\\ \"\\ abc\\ \"\\ )\\ 
% \n\\     [\\ \"\\ a\\ \"\\ , \\ \"\\ ab\\ \"\\ , \\ \"\\ abc\\ \"\\ ]\\ 
% \n\\      */\\ 
% \n\\     public List<String> allPrefixes(String string) {\\ 
% \end{tabular} &
% \begin{tabular}[c]{@{}l@{}}### Evaluation Rubric for the `allPrefixes` Function\\ \n
% **Score 1-3: Irrelevant or Nonsensical Responses**\\ \n
% - **1**: The response is completely unrelated to the prompt, providing code that does not even resemble a function to generate prefixes.\\ \n
% - **2**: The response contains some Java code, but it is nonsensical (e.g., using incorrect syntax or logic that does not relate to string manipulation).\\ \n
% - **3**: The response attempts to implement a function, but it fails to produce any output or the output is completely wrong (e.g., returns a fixed string or a number instead of a list of prefixes).\\ \n
% **Score 4-7: Incomplete or Flawed Implementations**\\ \n
% - **4**: The response includes a method that generates some prefixes but is missing key parts, such as returning the result or handling edge cases (e.g., does not handle an empty string).\\ \n
% - **5**: The response correctly implements a loop to generate prefixes but fails to include all necessary prefixes or returns them in the wrong order.\\ \n
% - **6**: The response generates prefixes correctly for some test cases but fails on others (e.g., works for \\ \"\\ abc\\ \"\\  but not for \\ \"\\ WWW\\ \"\\  or an empty string).\\ \n
% - **7**: The response is close to correct but contains minor issues, such as an off-by-one error or not using the correct return type, which leads to failing some test cases.\\ \n
% **Score 8-10: Mostly or Fully Correct Responses**\\ \n
% - **8**: The response correctly implements the logic to generate all prefixes and passes most test cases but may have a small inefficiency or stylistic issue (e.g., not using `List.of()` for static lists).\\ \n
% - **9**: The response is nearly perfect, correctly implementing the logic and passing all test cases but may have slight deviations from the canonical solution (e.g., using a different method for list creation).\\ \n
% - **10**: The response is fully correct, matches the canonical solution exactly, and passes all test cases without any issues, demonstrating a clear understanding of the problem and efficient implementation.
% \end{tabular} \\

% \midrule
% JavaScript &
% \begin{tabular}[c]{@{}l@{}}/* From a given list of integers, generate a list of rolling maximum element found until given moment\\ 
% \n\\   in the sequence.\\ 
% \n\\   >>> rollingMax([1, 2, 3, 2, 3, 4, 2])\\ 
% \n\\   [1, 2, 3, 3, 3, 4, 4]\\ 
% \n\\   */\\ 
% \n\\ const rollingMax = (numbers) => {\\ 
% \end{tabular} &
% \begin{tabular}[c]{@{}l@{}}### Evaluation Rubric for Rolling Maximum Function\\ \n
% #### Score 1-3: Irrelevant or Nonsensical Responses\\ \n
% - **1**: The response is completely irrelevant, such as returning a string or a different type of data structure (e.g., an object).\\ \n
% - **2**: The response shows an attempt to implement a function but does not reference the input list or the concept of rolling maximums (e.g., returns the sum of the list).\\ \n
% - **3**: The response includes some code structure but fails to utilize the input list correctly and does not implement any rolling maximum logic (e.g., a basic loop that does not update a maximum).\\ \n
% #### Score 4-7: Incomplete or Flawed Implementations\\ \n
% - **4**: The response attempts to implement the rolling maximum but has significant logical errors, such as not maintaining the maximum correctly throughout the iterations (e.g., only returns the maximum of the last element).\\ \n
% - **5**: The response partially implements the rolling maximum but fails on specific test cases. For example, it correctly handles the first few elements but fails to maintain the maximum as new elements are added.\\ \n
% - **6**: The response correctly processes the list but misses edge cases, such as returning incorrect results for lists with decreasing values or multiple equal maximums (e.g., returning a list that does not match expected outputs for some test cases).\\ \n
% - **7**: The response is close to correct but still has minor flaws in logic or edge cases, such as not handling an empty list correctly or returning the wrong maximum for specific sequences.\\ \n
% #### Score 8-10: Mostly or Fully Correct Responses\\ \n
% - **8**: The response implements the rolling maximum correctly for most test cases but fails on one specific edge case or does not handle empty lists properly.\\ \n
% - **9**: The response is nearly perfect, correctly implementing the rolling maximum logic and passing all test cases except for one minor edge case or inefficiency in the code (e.g., could be optimized further).\\ \n
% - **10**: The response fully aligns with the canonical solution, correctly implements the rolling maximum for all provided test cases, including edge cases, and efficiently handles the input list as specified in the prompt.
% \end{tabular} \\

% \midrule
% Python &
% \begin{tabular}[c]{@{}l@{}}def strlen(string: str) -> int:\\ 
% \n\\     \\ \"\"\"\\  Return length of given string\\ 
% \n\\     >>> strlen('')\\ 
% \n\\     0\\ 
% \n\\     >>> strlen('abc')\\ 
% \n\\     3\\ 
% \n\\     \\ \"\"\" 
% \end{tabular} &
% \begin{tabular}[c]{@{}l@{}}### Evaluation Rubric for `strlen` Function\\ \n
% **Score 1**: The response is irrelevant or nonsensical, providing code that does not relate to the prompt. For example, returning a fixed number or a string instead of an integer.\\ \n
% **Score 2**: The response attempts to define the function but fails to implement any logic that calculates the string length. For example, returning a placeholder value like `0` without using the input.\\ \n
% **Score 3**: The response includes a function definition but contains syntax errors or logical mistakes that prevent it from running. For example, using incorrect variable names or failing to return an integer.\\ \n
% ---\\ \n
% **Score 4**: The response defines the function and attempts to return the length of the string but uses an incorrect method. For example, using `string.size()` instead of `len(string)`.\\ \n
% **Score 5**: The response correctly implements the function but fails on one of the test cases. For example, it returns the correct length for an empty string and a single character but fails for longer strings.\\ \n
% **Score 6**: The response correctly implements the function and passes the test case for the empty string but fails on one additional test case, such as returning the wrong length for a string like 'abc'.\\ \n
% ---\\ \n
% **Score 7**: The response implements the function correctly using the `len` function but is not formatted or documented appropriately. It passes all test cases except possibly one. For example, it may return the correct length for 'x' and 'asdasnakj' but fails due to a minor error in the implementation.\\ \n
% ---\\ \n
% **Score 8**: The response is mostly correct and implements the function using `len(string)`. It passes the test cases provided in the prompt but may not handle edge cases or has minor issues in documentation or formatting.\\ \n
% **Score 9**: The response is correct and passes all test cases provided in the prompt, including the additional check cases. The implementation is clean and follows best practices, but may lack some documentation or edge case handling.\\ \n
% ---\\ \n
% **Score 10**: The response is fully correct, passing all test cases, including any additional checks. The implementation is concise, uses `len(string)` correctly, and includes appropriate documentation and comments, demonstrating a complete understanding of the prompt requirements.
% \end{tabular} \\

% \bottomrule
% \end{tabular}
% \caption{Example specific rubrics generated by the judge model.}
% \end{table}

